EvoAgent: Towards Automatic Multi-Agent Generation via Evolutionary Algorithms

The rise of powerful large language models (LLMs) has spurred a new trend in building LLM-based autonomous agents for solving complex tasks, especially multi-agent systems. Despite the remarkable progress, we notice that existing works are heavily dependent on human-designed frameworks, which greatly limits the functional scope and scalability of agent systems. How to automatically extend the specialized agent to multi-agent systems to improve task-solving capability still remains a significant challenge. In this paper, we introduce EvoAgent, a generic method to automatically extend specialized agents to multi-agent systems via the evolutionary algorithm, thereby improving the effectiveness of LLM-based agents in solving tasks. Specifically, we consider the existing agent frameworks as the initial individual and then apply a series of evolutionary operators (e.g., mutation, crossover, selection, etc.) to generate multiple agents with diverse settings. Experimental results across various tasks show that EvoAgent can significantly enhance the task-solving capability of LLM-based agents, and can be generalized to any LLM-based agent framework to extend them into multi-agent systems. Resources are available at https://evo-agent.github.io/.

==> list/autogen.tex <==

%\captionsetup[lstlisting]{position=bottom}
\begin{figure*}[htb]
\centering
\begin{minipage}{\textwidth}
\lstset{
    backgroundcolor=\color[RGB]{245,245,244},
    breaklines=true,
    breakindent=0pt,
    basicstyle=\ttfamily\small,
    emph={Expert,Specialized,Description,Interaction,Evaluation,Agent},
    emphstyle={\bfseries\color{NavyBlue}}
}\begin{lstlisting}[caption={An Illustration of \method's Adaptation to the AutoGen Framework},label=lst:ablation]

Specialized Agent Description: You are a historian with a deep understanding of British political history. Your expertise lies in the early 20th century, specifically the transition of power between Arthur Balfour and Henry Campbell-Bannerman. Your knowledge will be crucial in providing accurate and detailed information about this period, which will help to enrich the story's historical context.


Interaction:
user_proxy (to Historian):

Write a short and coherent story about Harry Potter that incorporates the answers to the following 5 questions: 
Who was the man behind The Chipmunks?
Which Lloyd Webber musical premiered in the US on 10th December 1993?
Who was the next British Prime Minister after Arthur Balfour?
Who had a 70s No 1 hit with Kiss You All Over?
What claimed the life of singer Kathleen Ferrier?
Answer:

Historian (to user_proxy):

Harry Potter and his friends, seated comfortably at a corner of the Gryffindor common room, were engrossed in a Muggle Studies project. Hermione, as usual, was leading the charge, but even she was puzzled by one question: "Who was the man behind The Chipmunks?" Harry was just as stumped, but Ron, after a long stare into the fire, smugly announced, "It was Ross Bagdasarian Sr., the chap who made them to sing in high-pitch voices."

The evening carried on, with the trio taking turns asking each other more about Muggle trivia to help with their project. Hermione next asked which Lloyd Webber musical premiered in the US on 10th December 1993. Ron, with his newfound confidence, erroneously suggested 'Cats', which left Hermione to correct him. "It was 'Sunset Boulevard', Ron. Always double-check your facts."

The next question had a touch of British political history. "Who was the next British Prime Minister after Arthur Balfour?" Harry, who had been mostly quiet, came alive. "It was Henry Campbell-Bannerman, right?" Hermione, clearly impressed, nodded in approval.

As they neared the end of their project, a new question came up - a Muggle music one. Ron, eager to redeem himself, asked: "Who had a 70s No 1 hit with 'Kiss You All Over'?" This time, Hermione seemed stumped. Harry, leafing through one of Hermione's Muggle music books, pointed out the answer. "It was Exile, a popular band in the 70s." For their final question, they took a rather somber turn. "What claimed the life of singer Kathleen Ferrier?" Hermione, looking sadly at a black and white photograph of the singer, answered softly. "Kathleen Ferrier was an incredibly talented contralto vocalist, tragically, she passed away from breast cancer."

At the end of the evening, the Gryffindor common room had once again proven to be a hub of knowledge - not just of magic, but also of Muggle trivia, political history, and even music. Harry, Hermione, and Ron, after an evening of exploration, felt even more connected to the Muggle world they so often strived to understand.

TERMINATE

Evaluation: correct_count=4/5
\end{lstlisting}
\end{minipage}\hfill
\begin{minipage}{\textwidth}
\end{minipage}
\end{figure*}

==> list/camel.tex <==

%\captionsetup[lstlisting]{position=bottom}
\begin{figure*}[htb]
\centering
\begin{minipage}{\textwidth}
\lstset{
    backgroundcolor=\color[RGB]{245,245,244},
    breaklines=true,
    breakindent=0pt,
    basicstyle=\ttfamily\small,
    emph={Expert,Description,Interaction,Evaluation,Agent},
    emphstyle={\bfseries\color{NavyBlue}}
}\begin{lstlisting}[caption={An Illustration of \method's Adaptation to the Camel Framework},label=lst:camel]

Specialized Agent Description: You are a historian with a deep understanding of British political history. Your expertise lies in the early 20th century, specifically the transition of power between Arthur Balfour and Henry Campbell-Bannerman. Your knowledge will be crucial in providing accurate and detailed information about this period, which will help to enrich the story's historical context.

Interaction:
[AI User] Instruction: Write a short story about Harry Potter that incorporates the answers to the following 5 questions:
1. Who was the man behind The Chipmunks?
2. Which Lloyd Webber musical premiered in the US on 10th December 1993?
3. Who was the next British Prime Minister after Arthur Balfour?
4. Who had a 70s No 1 hit with Kiss You All Over?
5. What claimed the life of singer Kathleen Ferrier?

Input: None.

[AI Assistant] Solution: 

As the new school year began at Hogwarts, whispers of a mysterious figure resembling Ross Bagdasarian Sr., the man behind The Chipmunks, spread throughout the wizarding community. Some claimed he had a knack for communicating with magical creatures, while others believed he possessed a secret talent for brewing potions unlike any seen before.

The students eagerly prepared for the annual Hogwarts musical, this year featuring "Joseph and the Amazing Technicolor Dreamcoat," the Lloyd Webber masterpiece that premiered in the US on 10th December 1993. The enchanting story of Joseph's journey captivated the audience, with spells and charms enhancing the magical performances on stage.

In the midst of magical rehearsals and academic studies, news arrived from the Muggle world that Sir Henry Campbell-Bannerman had succeeded Arthur Balfour as the British Prime Minister. The wizarding community closely followed the political developments, curious about the impact on their own world.

Meanwhile, a group of talented students formed a magical band inspired by the Muggle group Exile, who had a 70s No 1 hit with "Kiss You All Over." Their music echoed through the castle corridors, enchanting listeners with its catchy tunes and magical melodies.

Tragedy struck when a beloved singing sensation, Kathleen Ferrier, succumbed to breast cancer, a devastating loss felt deeply by both the Muggle and wizarding communities. Her hauntingly beautiful voice would forever be remembered, a reminder of the fragility of life and the power of music to transcend boundaries.

As the school year progressed, Harry Potter and his friends navigated a world where magic and history intertwined, learning valuable lessons about courage, friendship, and the enduring legacy of those who came before them.

Evaluation: correct_count=3/5
\end{lstlisting}
\end{minipage}\hfill
\begin{minipage}{\textwidth}
\end{minipage}
\end{figure*}

==> list/ea.tex <==

%\captionsetup[lstlisting]{position=bottom}
\begin{figure*}[htb]
\centering
\begin{minipage}{\textwidth}
\lstset{
    backgroundcolor=\color[RGB]{245,245,244},
    breaklines=true,
    breakindent=0pt,
    basicstyle=\ttfamily\small,
    emph={Step,One,Two},
    emphstyle={\bfseries\color{NavyBlue}}
}\begin{lstlisting}

Step One: Generate the initial population of individuals randomly. 
Step Two: Execute the following re-generational steps until termination:
   1. Evaluate the fitness of each individual in the population.
   2. Select the fittest individuals for reproduction.
   3. Create new individuals through crossover and mutation operations.
   4. Update the individuals in the population with new ones.

\end{lstlisting}
\end{minipage}\hfill
\begin{minipage}{\textwidth}
\end{minipage}
\end{figure*}

==> list/metagpt.tex <==

%\captionsetup[lstlisting]{position=bottom}
\begin{figure*}[htb]
\centering
\begin{minipage}{\textwidth}
\lstset{
    backgroundcolor=\color[RGB]{245,245,244},
    breaklines=true,
    breakindent=0pt,
    basicstyle=\ttfamily\small,
    emph={Expert,Description,Interaction,Evaluation,Debate,Topic,Original,Role},
    emphstyle={\bfseries\color{NavyBlue}}
}\begin{lstlisting}[caption={An Illustration of \method's Adaptation to the MetaGPT Framework},label=lst:ablation]

Debate Topic: The U.S. should commit more in climate change fighting

Original Role:
- Biden: Democrat
- Trump: Republican

Original Interaction:
Biden: Ladies and gentlemen, we are at a pivotal moment. While my opponent denies the urgency of climate change, I stand with science. We must act boldly to secure a sustainable future for our children and grandchildren. Investing in clean energy not only addresses the climate crisis but also creates jobs and strengthens our economy. We cannot afford to ignore reality. The cost of inaction is far too high. It's time to lead, not to lag. Let's choose hope over fear, and action over denial.

Trump: Ladies and gentlemen, the real crisis is the economic disaster under Biden's policies. He talks about investments, but it's your tax dollars he's spending. We need reliable, affordable energy, not expensive fantasies. Under my administration, we achieved energy independence and booming job growth. Biden's plan will kill jobs and increase dependency on foreign energy. We can't let that happen. Let's prioritize American workers and realistic solutions, not scare tactics and wasteful spending. Let's make America great again!

Biden: Ladies and gentlemen, my opponent's vision is shortsighted. We're not just investing in clean energy; we're investing in America's future. These aren't fantasies; they're opportunities for sustainable, high-paying jobs right here at home. Under my plan, we won't just match the job growth of the past; we'll exceed it. We're building an economy that's resilient, green, and forward-thinking. We cannot afford to return to policies that ignore science and jeopardize our children's future. Let's build back better, responsibly.

Trump: Ladies and gentlemen, Biden's plan is a disaster wrapped in good intentions. He promises jobs, but at what cost? His green dreams are funded by your hard-earned dollars, leading to higher taxes and energy costs. We can't gamble our economy on unproven technologies. Under my leadership, we saw real growth, not just promises. We need practical solutions, not pie-in-the-sky policies. Let's protect our economy and keep America strong and independent. Let's not just build back, let's build back smarter!

(Both debators have become entrenched in the same argument without presenting any compelling new evidence.)

\end{lstlisting}
\end{minipage}\hfill
\begin{minipage}{\textwidth}
\end{minipage}
\end{figure*}

==> table/agentframe.tex <==
% Table generated by Excel2LaTeX from sheet 'Sheet1'

%\begin{wraptable}{r}{0.4\linewidth}
\begin{table}[t]
\small
\caption{Comparison of \method with human-designed agent frameworks in Logic Grid Puzzle, Trivia Creative Writing tasks.}
\vspace{0.15cm}
  \centering
    \begin{tabular}{lcc}
    \toprule
    \textbf{Framework} & \textbf{Logic} & \textbf{Writing} \\
    \midrule
    \method & 77.00 & 84.40 \\
    AgentVerse & 66.50 & - \\
    AutoAgents & - & 82.00 \\
    \bottomrule
    \end{tabular}%
  \label{tab:framework}%
%\end{wraptable}
\end{table}

==> table/metagpt.tex <==

\begin{table}[t]
\footnotesize
  \centering
    \begin{tabularx}{\linewidth}{X}
    \toprule
    \rowcolor[gray]{0.95}\multicolumn{1}{c}{\textbf{I: Original MetaGPT Framework}} \\
    \midrule
    \makecell[l]{
    \textbf{Debate Topic:} The U.S. should commit more in climate change fighting\\
    \textbf{Original Role:} 1. Biden: Democrat 2. Trump: Republican\\
    %\textbf{Original Interaction:}\\
    \textbf{Round 1:}\\
    \textbf{Biden:} Ladies and gentlemen, we are at a pivotal moment. While my opponent denies the urgency of climate \\ change, I stand with science. We must act boldly to secure a sustainable future for our children and \\ grandchildren. Investing in clean energy not only addresses the climate crisis but also creates jobs and \\ strengthens our economy. We cannot afford to ignore reality. The cost of inaction is far too high. It's time to \\lead, not to lag. Let's choose hope over fear, and action over denial.\\
    \textbf{Trump:} Ladies and gentlemen, the real crisis is the economic disaster under Biden's policies. He talks about \\ investments, but it's your tax dollars he's spending. We need reliable, affordable energy, not expensive fantasies. \\ Under my administration, we achieved energy independence and booming job growth. Biden's plan will kill\\ jobs and increase dependency on foreign energy. We can't let that happen. Let's prioritize American workers \\and realistic solutions, not scare tactics and wasteful spending. Let's make America great again!\\
    \textbf{Round 2:}\\
    \textbf{Biden:} Ladies and gentlemen, my opponent's vision is shortsighted. We're not just investing in clean energy;\\ we're investing in America's future. These aren't fantasies; they're opportunities for sustainable, high-paying\\ jobs right here at home. Under my plan, we won't just match the job growth of the past; we'll exceed it. We\\ are building an economy that's resilient, green, and forward-thinking. We cannot afford to return to policies \\that ignore science and jeopardize our children's future. Let's build back better, responsibly.\\
    %...\\
    %\textbf{Trump:} Ladies and gentlemen, Biden's plan is a disaster wrapped in good intentions. He promises jobs, but\\ at what cost? His green dreams are funded by your hard-earned dollars, leading to higher taxes and energy\\ costs. We can't gamble our economy on unproven technologies. Under my leadership, we saw real growth,\\ not just promises. We need practical solutions, not pie-in-the-sky policies. Let's protect our economy and keep \\America strong and independent. Let's not just build back, let's build back smarter!
    }\\
    
    \midrule
    
    \rowcolor[gray]{0.95}\multicolumn{1}{c}{\textbf{II: Multi-agent Generation for MetaGPT Framework}} \\
    \midrule
    \makecell[l]{
    \textbf{Round 1:}\\
    \textbf{Expert 1 for Democrat}: You are a historian specializing in U.S. environmental policy. As such, you  \\ are tasked with ensuring the arguments stand the test of historical accuracy. Utilize your knowledge in the \\ history of environmental policy and debates in the U.S. to cross-check the statements made and identify any \\historical events or legislations that support the assertions. Find instances where ignoring environmental \\ issues led to disastrous consequences.\\% Also, highlight how previous administrations have addressed climate \\ change and the results of their actions. This will help formulate a stronger, historically-supported argument.\\
    \textbf{Expert 1 for Republican}: You are an economist with a specialization in environmental economics. \\With your deep understanding of cost-benefit analyses, assess the potential economic implications of \\environmental regulations like the Clean Air Act and the Paris Agreement. Evaluate their effects on businesses,\\ jobs, and overall economic growth. Provide insight into how technological innovation can offer economic \\advantages while also considering environmental protection.\\% Your involvement in this discussion will ensure\\ the soundness and verifiability of the economic arguments stated.\\
    \textbf{Biden (Revised):} Ladies and gentlemen, the Dust Bowl of the 1930s should serve as a poignant reminder of \\the dire consequences of environmental neglect. Embracing regulations like the Clean Air Act has proven to be\\ beneficial for both human health and economy. Our participation in global efforts, such as the Paris Agreement, \\underscores our commitment to taking decisive action. Investing in clean energy is not only a step towards \\climate resilience, but also a catalyst for job creation and economic fortification. Let's act now to prevent \\another catastrophic environmental disaster.\\
    \textbf{Trump (Revised):} We wholeheartedly agree on preventing environmental catastrophes, but we must balance \\this with the economic realities in play. While the Clean Air Act and the Paris Agreement show ambitious\\ environmental commitment, their economic burden on American businesses and jobs lead to a challenging \\transition. We must strategize on efficient, sustainable, and fiscally responsible transitions. This involves \\harnessing technology and innovation, creating a balance between economic growth and environmental \\preservation. We must aspire for a strong, independent, and prosperous America while ensuring we act\\ prudently on our environment.\\
    \textbf{Round 2:}\\
    \textbf{Expert 2 for Democrat}: You are a climate scientist with a deep understanding of climate change and its \\impacts. Use your expertise to provide accurate information about the consequences of inaction on climate\\ change. Highlight the long-term effects it can have on our planet's health, such as extreme weather and health \\crises, and provide scientifically-backed evidence to support these points. Furthermore, discuss the potential \\benefits of the proposed clean energy initiatives on the environment.\\
    \textbf{Expert 2 for Republican}: You are a political strategist experienced in public policy and communication. \\Utilize your expertise in framing arguments that resonate with different voter demographics while focusing on\\ Trump's stance. Analyse the merits in what Biden's arguments offer and guide on how best to counter these \\points without dismissing the underlying concern which is climate change.\\
    \textbf{Biden (Revised):} Mr. Trump, while I respect your attention to economic realities, we must not lose sight of\\ our planet's long-term health, which is intrinsically tied to our economy. Climate science indicates that inaction\\ will lead to extreme weather, health crises, and biodiversity loss. These potential outcomes present significantly\\ more expensive scenarios than the transition cost you mention. Clean energy presents an economic opportunity.\\ Jobs in this sector are growing rapidly, offering a path to a thriving economy built on sustainable foundations.\\ It's not just about convenience—it's about responsible stewardship.\\
    %\textbf{Trump (Revised):} Mr. Biden, we wholeheartedly agree on preventing environmental catastrophes, but we \\must balance this with the economic realities in play. While the Clean Air Act and the Paris Agreement show \\ambitious environmental commitment, their economic burden on American businesses and jobs lead to a \\challenging transition. We must strategize on efficient, sustainable, and fiscally responsible transitions. This \\involves harnessing technology and innovation, creating a balance between economic growth and environmental\\ preservation. We must aspire for a strong, independent, and prosperous America while ensuring we act\\ prudently on our environment.
     }\\
    \bottomrule
    \end{tabularx}
  \caption{An Illustration of \method's Adaptation to the MetaGPT Framework.
  }
  \label{tab:instruction_prompt}
\end{table}
